Compositional Learning of Image-Text Query for Image Retrieval

In this paper, we investigate the problem of retrieving images from a database based on a multi-modal (image-text) query. Specifically, the query text prompts some modification in the query image and the task is to retrieve images with the desired modifications. For instance, a user of an E-Commerce platform is interested in buying a dress, which should look similar to her friend's dress, but the dress should be of white color with a ribbon sash. In this case, we would like the algorithm to retrieve some dresses with desired modifications in the query dress. We propose an autoencoder based model, ComposeAE, to learn the composition of image and text query for retrieving images. We adopt a deep metric learning approach and learn a metric that pushes composition of source image and text query closer to the target images. We also propose a rotational symmetry constraint on the optimization problem. Our approach is able to outperform the state-of-the-art method TIRG \cite{TIRG} on three benchmark datasets, namely: MIT-States, Fashion200k and Fashion IQ. In order to ensure fair comparison, we introduce strong baselines by enhancing TIRG method. To ensure reproducibility of the results, we publish our code here: \url{https://github.com/ecom-research/ComposeAE}.

==> MIT-States.tex <==
\begin{table}
\centering
\begin{tabular}{|l|ccc|}
\hline
Method & R@1 & R@5 & R@10\\
\hline\hline
% Image only & 3.3$^{\pm0.1}$ & 12.8$^{\pm0.2}$ & 20.9$^{\pm0.1}$\\
% Text only & 7.4$^{\pm0.4}$ & 21.5$^{\pm0.9}$ & 32.7$^{\pm0.8}$\\
%\hline
% PM -- projection module
% Concatenation & 11.8$^{\pm0.2}$ & 30.8$^{\pm0.2}$ & 42.1$^{\pm0.3}$ \\
Show and Tell & 11.9$^{\pm0.1}$ & 31.0$^{\pm0.5}$ & 42.0$^{\pm0.8}$ \\
Att. as Operator  & 8.8$^{\pm0.1}$ & 27.3$^{\pm0.3}$ & 39.1$^{\pm0.3}$ \\
Relationship  & 12.3$^{\pm0.5}$ & 31.9$^{\pm0.7}$ & 42.9$^{\pm0.9}$ \\
FiLM  & 10.1$^{\pm0.3}$ & 27.7$^{\pm0.7}$ & 38.3$^{\pm0.7}$ \\
TIRG & 12.2$^{\pm0.4}$ & 31.9$^{\pm0.3}$ & 43.1$^{\pm0.3}$\\
\hline

TIRG with BERT & {12.3}$^{\pm0.6}$ & {31.8}$^{\pm0.3}$ & {42.6}$^{\pm0.8}$  \\
TIRG with &  &  & \\ Complete Text Query & 7.9$^{\pm 1.9}$ & 28.7$^{\pm 2.5}$ & 34.1$^{\pm2.9}$  \\
% TIRG with &  &  & \\ Complete Text Query & 12.9$^{\pm 0}$ & 33.7$^{\pm 0}$ & 44.1$^{\pm0}$  \\
% runs TIRG with complete text query 54k iterations
% r1: 0.03714, 0.05374
% r5: 0.11, 0.1752
% r10: 0.1781, 0.2511
\hline

TIRG with BERT and &&&\\ Complete Text Query & \underline{13.3}$^{\pm0.6}$ & \underline{34.5}$^{\pm1.0}$ & \underline{46.8}$^{\pm1.1}$ \\
% & 13.6$^{\pm0.9}$  & 35.5$^{\pm0.8}$  & 47.4$^{\pm1.1}$  \\
% saturated 66k: & {13.3}$^{\pm0.6}$ & {34.5}$^{\pm1.0}$ & {46.8}$^{\pm1.1}$ 
\hline
ComposeAE & \textbf{13.9}$^{\pm0.5}$ & \textbf{35.3}$^{\pm0.8}$ & \textbf{47.9}$^{\pm0.7}$\\ %https://workflowy.com/#/e9f3c5bb2d4a % ...

\hline
\end{tabular}
% \vspace{3mm}
\caption{Model performance comparison on MIT-States. The best number is in bold and the second best is underlined.}
\label{tab:mitstates}
\end{table}


==> f200k.tex <==

\begin{table}[ht]

\centering

% \resizebox{0.9}
{\begin{tabular}{|l|ccc|}
\hline
Method & R@1 & R@10 & R@50 \\
\hline\hline
Han \etal~\cite{han2017automatic}  & 6.3 & 19.9 & 38.3 \\
% Image only & 3.5 & 22.7 & 43.7 \\
% Text only & 1.0 & 12.3 & 21.8 \\
%\hline
% Concatenation & 11.9$^{\pm1.0}$ & 39.7$^{\pm1.0}$ & \underline{62.6}$^{\pm0.7}$ \\
Show and Tell & 12.3$^{\pm1.1}$ & 40.2$^{\pm1.7}$ & 61.8$^{\pm0.9}$ \\
Param Hashing & 12.2$^{\pm1.1}$ & 40.0$^{\pm1.1}$ & 61.7$^{\pm0.8}$ \\
Relationship & {13.0}$^{\pm0.6}$ & {40.5}$^{\pm0.7}$ & 62.4$^{\pm0.6}$ \\
FiLM  & 12.9$^{\pm0.7}$ & 39.5$^{\pm2.1}$ & 61.9$^{\pm1.9}$ \\
TIRG & {14.1}$^{\pm0.6}$ & {42.5}$^{\pm0.7}$ & {63.8}$^{\pm0.8}$ \\
\hline
TIRG with BERT & 14.2$^{\pm1.0}$ & 41.9$^{\pm1.0}$ & 63.3$^{\pm0.9}$  \\
TIRG with &  &  & \\ Complete Text Query & 18.1$^{\pm1.9}$ & \underline{52.4}$^{\pm2.7}$ & \underline{72.1}$^{\pm2.1}$  \\
% TIRG with &  &  & \\ Complete Text Query & 18.1$^{\pm0}$ & 47.4$^{\pm0}$ & 69.8$^{\pm0}$  \\
% runs TIRG with complete text query 59k iterations
% r1: 0.1779, 0.1547, 0.1797
% r10: 0.5546, 0.482, 0.512
% r50: 0.7418, 0.7767, 0.7535

\hline
TIRG with BERT and &  &  & \\ Complete Text Query & \underline{19.9}$^{\pm1.0}$ & {51.7}$^{\pm1.5}$ & {71.8}$^{\pm1.3}$  \\
\hline
ComposeAE & \textbf{22.8}$^{\pm0.8}$ & \textbf{55.3}$^{\pm0.6}$ & \textbf{73.4}$^{\pm0.4}$ \\
\hline
\end{tabular}}

\label{tab:f200k}
% \vspace{3mm}
\caption{Model performance comparison on Fashion200k. The best number is in bold and the second best is underlined.}
\end{table}


==> fiq.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.89\linewidth]{FIQ_Retrieval.jpg}
\caption{Qualitative Results: Retrieval examples from FashionIQ Dataset}
\label{fig:fIQqual}
\end{figure*}


\begin{table}[ht]

\centering
\begin{tabular}{|l|ccc|}
\hline
Method & R@10 & R@50 & R@100 \\
\hline\hline
TIRG with &  &  & \\ Complete Text Query & 3.34$^{\pm0.6}$  & 9.18$^{\pm0.9}$  &  9.45$^{\pm0.8}$ \\
% saturated 17k: & {3.4}$^{\pm0.7}$ & {9.1}$^{\pm0.6}$ & {9.11}$^{\pm0.6}$ 
\hline
TIRG with BERT and &  &  & \\ Complete Text Query & \underline{11.5}$^{\pm0.8}$ & \underline{28.8}$^{\pm1.5}$ & \underline{28.8}$^{\pm1.6}$
% saturated 17k: & {11.5}$^{\pm0.7}$ & {28.8}$^{\pm1.5}$ & {28.8}$^{\pm1.6}$ 
\\
\hline
ComposeAE & \textbf{11.8}$^{\pm0.9}$ & \textbf{29.4}$^{\pm1.1}$ & \textbf{29.9}$^{\pm1.3}$ \\

\hline
\end{tabular}

\label{tab:fiq}
\vspace{3mm}
\caption{Model performance comparison on Fashion IQ. The best number is in bold and the second best is underlined.}
\end{table}


% We can see that both TIRG variants are not able to form a good embedding to rank candidates when some of the target images haven't seen by the algorithm in the training phase as a source image. That makes TIRG approach less efficient and both for R@50 and R@100 we see essentially the same performance. That proves the fact that the search in multi-modal must not only be based on the rich context representation (which is provided by BERT) but should not weaken the text feature contribution.

% The main difference between experiments on Fashion-IQ and two other datasets is that in former the algorithm is supposed to rank and retrieve images which haven't seen by the algorithm in the training pipeline just by using the text query. In two other datasets, in the way they have been constructed lies an implicit bias: a small vocabulary and short number of transitions between each of the objects. That's why in the wildest of conditions when both the image domain is the same for all images and text description is fairly complex (case for fashion200k and fashionIQ, not MITStates) and the inference runs on the unknown images which haven't been in train, TIRG appoarch fails to place similar images together in high-dimensional ranking space. Firstly, because of the failing in providing a complex context embedding with TIRG original LSTM and secondly, not able to correctly place the images in the space having the complex context embedding provided by BERT (because of not treating the text feature properly).

% Sidenotes:

% I guess we should focus on the idea that it is necessary to provide a rich text embedding in order to learn a rich multi-modal representation and the learned multi-modal representation should possess the properties we constraint it within the solution space as you wrote above in the paper.
